LLM-SQL-Solver: Can LLMs Determine SQL Equivalence?

Judging the equivalence between two SQL queries is a fundamental problem with many practical applications in data management and SQL generation (i.e., evaluating the quality of generated SQL queries in text-to-SQL task). While the research community has reasoned about SQL equivalence for decades, it poses considerable difficulties and no complete solutions exist. Recently, Large Language Models (LLMs) have shown strong reasoning capability in conversation, question answering and solving mathematics challenges. In this paper, we study if LLMs can be used to determine the equivalence between SQL queries under two notions of SQL equivalence (semantic equivalence and relaxed equivalence). To assist LLMs in generating high quality responses, we present two prompting techniques: Miniature & Mull and Explain & Compare. The former technique is used to evaluate the semantic equivalence in which it asks LLMs to execute a query on a simple database instance and then explore if a counterexample exists by modifying the database. The latter technique is used to evaluate the relaxed equivalence in which it asks LLMs to explain the queries and then compare if they contain significant logical differences. Our experiments demonstrate using our techniques, LLMs is a promising tool to help data engineers in writing semantically equivalent SQL queries, however challenges still persist, and is a better metric for evaluating SQL generation than the popular execution accuracy.

==> ICDEsections/mainresults.tex <==
\section{Evaluations}
\label{sec:eval}
We evaluate the capabilities of popular large language models in identifying semantic and pragmatic equivalence between a pair of SQL queries. In particular, we aim to answer the following questions: 
\begin{itemize}
    \item Is the Miniature \& Mull prompt effective in accurately determining semantic equivalence?

    \item Does LLMs using the Explain \& Compare prompt achieve better alignment with human preferences than execution match?
    
\end{itemize}

We showcase the experimental results using  the popular GPT-3.5-Turbo (gpt-3.5-turbo) and GPT-4o (gpt-4o) models. The models are accessed via OpenAI API.

\textbf{Hyper-parameter:} In the API call for all experiments, we have set temperature to 0 which implies greedy sampling is used to generate the output; The max tokens are set to 4096.

\textbf{Few shot demonstrations.} In addition to the zero-shot setting, we also investigate the in-context learning capabilities of LLMs in determining SQL equivalence. This is achieved by providing five static few-shot examples as part of the input context to guide the model's reasoning process. For the semantic equivalence, the five static examples include three semantically equivalent SQL queries and two semantically inequivalent SQL queries. Similarly, for pragmatic equivalence, the five static examples consist of three equivalent and two inequivalent query pairs. The equivalent examples feature queries that share the same intent despite differences in their structure. For instance, queries like "SELECT birth\_country FROM player" and "SELECT birth\_city FROM player" are considered equivalent as both aim to determine the birth location, albeit at different levels of granularity.

\subsection{Data Source}


\textcolor{black}{First, we compare our proposed \textit{Miniature \& Mull} prompt with the CoT prompt on i) Calcite test suites~\cite{begoli2018apache, ding2023proving} and ii) Inequivalent Queries~\cite{gao2023text}}. \textcolor{black}{These two data sources include pairs of SQL queries that have been expertly labeled as semantically equivalent or non-equivalent.} 

Next, we present the results evaluating the alignment between our proposed LLM-SQL-Solver's pragmatic equivalence judgments and human preferences. To conduct this assessment, we selected 70 pairs of SQL queries, comprising gold-standard SQL queries from the Spider benchmark~\cite{yu2018spider} and predicted SQL queries generated by LLMs~\cite{gao2023text, pourreza2023din, liu2023comprehensive}. Each SQL pair was independently reviewed and labeled by at least three human experts proficient in SQL. The final label for each pair was determined through a majority voting process, ensuring consensus among the reviewers. This approach provides a robust benchmark for comparing the LLM's pragmatic equivalence evaluations with human judgment. In addition to the human preference, we also provide the execution accuracy (EX) by executing these 70 queries over Spider databases. In all experiments, we use the open sourced EX evaluation code from GitHub~\footnote{https://github.com/THU-BPM/ChatGPT-sql}. 

% The Spider benchmark contains 1034 development questions covering 20 databases in different domains. The Spider SQL queries are classified into four levels of complexity: easy, medium, hard, and extrahard (extra).

% The non-equivalent queries are first used to evaluate the performance of Cosette a formal language based SQL solver; however, Cosette does not support many SQL operations, such as \textit{IN} and \textit{EXCEPT}, and the Cosette project is no longer maintained. \textcolor{black}{The equivalent queries, comprising pairs of gold SQL queries from the Spider benchmark~\cite{yu2018spider} and model predictions, are manually analyzed in~\cite{zhong2020semantic}.}

% We use Nonequivalent Queries to investigate if LLMs can successfully notice the semantic differences (often subtle) between two non-equivalent SQL queries.
\begin{itemize}

    \item \textbf{Calcite test suites}: It contains 232 pairs of equivalent queries (verified by expert) in the Calcite test suites.
    
    \item \textbf{Semantically Inequivalent Queries}: It contains 180 pairs of semantic inequivalent queries. One of the query is the gold SQL in spider benchmark~\cite{yu2018spider} and the other is a predicted SQL query from DAIL-SQL~\cite{gao2023text}. Because they have different execution outputs, the databases in spider benchmark serve as counter examples.


    \item \textbf{Pragmatic Equivalence Queries}: It contains 70 pairs of SQL queries with human preference label. Each pair has been independently reviewed and labeled by at least three human experts to capture human preference judgments.
    
\end{itemize}

% This classification is based on various factors, including the quantity of SQL keywords utilized, the incorporation of nested sub queries, and the usage of column selections and aggregations. 

% % Since equivalent SQL queries can be written in many different ways, execution accuracy (EX) is commonly used as the metrics. 
% \begin{itemize}
%     \item \textbf{Chat}~\cite{liu2023comprehensive}: Generate queries using ChatGPT with the zero-shot basic prompt.
    
%     \item \textbf{DIN}~\cite{pourreza2023din}: Generate SQL queries by decomposing the task into fine grained sub-modules and use the GPT-4 model with few-shot prompting.
    
%     \item \textbf{DAIL}~\cite{dail_sql}: The current SOTA open sourced technique on the Spider benchmark. It uses the GPT-4 model with few-shot prompting and incorporates self-consistency~\cite{wang2022self}.
% \end{itemize}

\subsection{Judging Semantic Equivalence}

\begin{table*}[tbph]
    \centering
    \caption{Results in determining semantic equivalent and non-equivalent queries for GPT-3.5-Turbo (ChatGPT) and GPT-4o across different prompting strategies (CoT and M\&M) in zero-shot and few-shot settings.}
    \renewcommand{\arraystretch}{1.5} % Adjust row height
    \setlength{\tabcolsep}{10pt} % Adjust column width
    \begin{tabular}{l|l|c|c|c|c}
        \hline
        {\bf Judge} & {\bf Prompt} & \multicolumn{2}{c|}{\bf Semantic Eq. } & \multicolumn{2}{c}{\bf Semantic Ineq. } \\
        \cline{3-6}
        & & {\bf 0-Shot} & {\bf 5-Shot} & {\bf 0-Shot} & {\bf 5-Shot} \\
        
        \hline
        \multirow{2}{*}{ChatGPT} 
        & CoT & 53\% & 52\% & 63\% & 46\% \\ \cline{2-6}
        
        & M\&M & 85\% (+32\%) & 87\% (+35\%) & 67\% (+4\%) & 47\% (+1\%) \\ \hline
        
        \multirow{2}{*}{GPT-4o} 
        & CoT & 81\% & 83\% & 85\% & 83\% \\ \cline{2-6}
        & M\&M & 84\% (+3\%) & 89\% (+6\%) & 86\% (+1\%) & 85\% (+2\%) \\ \hline
    \end{tabular}
    \label{tab:semantic}
\end{table*}



Recall that two queries cannot be semantically equivalent if there exists a counter example (a database instance) such that two queries produce different outputs. We used two different prompting methods \textit{CoT} and \textit{Miniature \& Mull} to compare and contrast the accuracy of LLMs in determining semantic equivalence.



 % GPT 4 Turbo failed to notice the subtle difference in the COUNT BUG, whereas GPT 3.5 Turbo correctly output that queries in COUNT BUG are not semantically equivalent. In addition, 

% Therefore, we operate under the assumption that the underlying database instance is case-insensitive when evaluating semantic equivalence.



As shown in Table~\ref{tab:semantic}, we can observe that the \textit{Miniature \& Mull} prompt always provides a higher accuracy than the \textit{CoT} prompt. For determining the semantic equivalent queries (Calcite test suite), \textit{Miniature \& Mull} prompt using GPT-4o achieved around 90\% accuracy. For determining the semantic inequivalent queries (DAIL-SQL results over Spider Benchmark), \textit{Miniature \& Mull} prompt using GPT-4o achieved around 86\% accuracy. We can also observe that when using the weaker GPT-3.5-Turbo in judging semantically equivalent queries,  \textit{Miniature \& Mull} outperform \textit{CoT} prompt (asking LLMs to determine SQL equivalence and think step by step) by more than 30\%. However, when judging the inequivalent SQL queries, we find that the GPT-3.5-Turbo significantly under-perform than the GPT-4o Turbo model. 

Analyzing responses for identifying SQL-inequivalent queries, we observed a few reasons for GPT-3.5-Turbo's low accuracy:
\begin{enumerate}
    \item Distinct entries vs duplicated entries. GPT-3.5-Turbo often failed to consider the difference between selecting unique rows and selecting rows that may be duplicated.
    
    \item Case-Sensitivity Ignored: GPT-3.5-Turbo often disregards the fact that the database is \textbf{case-sensitive}. Althought we have explicitly noted the database is string case-sensitive in the prompt, GPT-3.5-Turbo often fails to strictly adhere to the case-sensitivity requirement, resulting in inaccuracies when comparing queries. This observation aligns with findings in prior work~\cite{wen2024benchmarking}, which highlight GPT-3.5-Turbo's challenges in reliably following instructions compared to stronger models such as GPT-4o.

    \item 
    Overlooked Subtle Differences: GPT-3.5-Turbo may also fail to detect critical differences in column and table names. For instance, it might incorrectly treat distinct column names as equivalent or overlook the inclusion of additional columns or elements in a query. A specific example includes comparing \textit{AVG(capacity)} with \textit{avg\_capacity}, where the former performs an average operation on the \textit{capacity} column, while the latter refers to an entirely different column. Similarly, in cases like \textit{GROUP BY id} versus \textit{GROUP BY student\_id}, GPT-3.5-Turbo may fail to recognize these distinctions, potentially leading to incorrect judgments.

    \item Hallucination. In the \textit{Miniature \& Mull} prompt, LLMs are instructed to execute both SQL queries on a simple database they create and then repeat the process on a modified version of the database to compare outputs. GPT-3.5-Turbo often returns incorrect results when executing SQL queries on its self-generated database instances. Moreover, even when the outputs are identical, it may mistakenly assert that the results differ. This hallucination and the resulting snowballing effect~\cite{zhang2023language} significantly contribute to GPT-3.5-Turbo's poorer performance compared to GPT-4o.
    
\end{enumerate}

When GPT-4o is used to determine SQL semantic equivalence, it consistently produces more accurate and reliable decisions for both equivalent and inequivalent queries. A notable observation is that GPT-4o reliably identifies the distinction between \textit{ORDER BY ASC/DESC LIMIT 1} and \textit{WHERE col = (SELECT MIN/MAX(col))}. The former always returns a single row due to the \textit{LIMIT 1} clause, whereas the latter may return multiple rows if several share the same minimum or maximum value. This critical difference is often overlooked by GPT-3.5-Turbo. When using the \textit{CoT} (Chain-of-Thought) prompt, GPT-4o achieves an accuracy of 82\% – 85\%, and with the \textit{Miniature \& Mull} prompt, it improves further to 85\% – 90\%.

Furthermore, we observe that, in general, adding few-shot demonstrations improves accuracy. However, for semantically inequivalent queries, incorporating the five static examples results in a significant drop in accuracy for both the \textit{CoT} and \textit{Miniature \& Mull} prompts when using GPT-3.5-Turbo. The same few shot approach leads to only a slight accuracy decline when using GPT-4o. 
This discrepancy underscores the superior in-context learning capabilities of GPT-4o compared to GPT-3.5-Turbo. GPT-4o demonstrates a greater ability to interpret and generalize from the provided examples, enabling it to more effectively account for nuanced differences in semantic meaning. Conversely, GPT-3.5-Turbo struggles with leveraging the few-shot examples for semantically inequivalent queries, likely due to limitations in its contextual reasoning and pattern recognition abilities. This results in a diminished capacity to differentiate between queries with subtle semantic differences. Moreover, we believe that determining SQL semantic equivalence is an inherently challenging task for LLMs. It requires an understanding of both the syntax and the underlying logic of the queries. While few-shot learning provides valuable context, it may not always suffice to overcome the complexities involved, particularly for cases where the differences between queries are subtle or deeply tied to specific database schema (e.g., Primary Key and Foreign Key relationships).

Despite the aforementioned challenges in determining SQL semantic equivalence, our proposed \textit{Miniature \& Mull} prompt always achieve higher accuracy than using \textit{Cot} prompt. This demonstrates the effectiveness of our approach in addressing some of the inherent difficulties of the task. As a result, we believe that letting LLMs execute SQL queries on a simple database instance and then assessing whether a counterexample can be generated by modifying the database is a more effective method to determine SQL semantic equivalence. 

To conclude this subsection, we also note that there are a few very rare cases that we observed in which the SQL queries are semantically equivalent but execution match determines not equivalent. For example, when the provided database in Spider contains column values that can not be decoded (similar issues are also raised~\cite{spiderissue}, semantically equivalent queries can be misclassified by execution match but very rare. 

% GPT 4 Turbo failed on a user found bug originally posted on Hackers News~\cite{hackernews}. 
% This bug contains two SQL queries where one used \textit{DISTINCT} in selection and the other used \textit{UNION ALL} to union two sub-queries. Hence, GPT 4 Turbo failed to recognize that \textit{UNION ALL} will not remove duplicate rows (though \textit{UNION} will). GPT 3.5 Turbo failed on the CSE344 exam question which involves different sub-queries. When using \textit{Miniature \& Mull} (asking LLMs to first run a simple example over the given SQL queries and then examining if the example database can be modified to generate a counter example), GPT 3.5 Turbo and GPT 4 Turbo both successfully identified all the mistakes. 



% Moreover, since GPT 4 Turbo showcases strong performance with faster response time, we use GPT 3.5 Turbo and GPT 4 Turbo for all the following experiments.

% We can observe that, when using \textit{Counter Example} prompt (follows the main ideas of chain of thoughts), LLMs scores at least 60\% accuracy. When using the \textit{Miniature \& Mull} prompting, the accuracy is significantly improved to 100\% for GPT 3.5 Turbo and GPT 4 Turbo. 
\begin{table*}[tbph]
    \centering
    \caption{A breakdown of the accuracy scores when using different metrics, i.e., EX and LLMs' judgments. The LLMs' judgments uses \textit{Explain \& Compare} prompt with five static demonstrations. The compared SQL queries are the gold SQL queries from Spider and the generated SQL queries from Chat-SQL, DIN-SQL, and DAIL-SQL.}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l||l|l l l l l l}\hline
        {\bf Judge} & {\bf Data} & {\bf Easy} & {\bf Medium} & {\bf Hard} & {\bf Extra} & {\bf Overall Acc} & {\bf Rank} \\ \hline
        \hline
        - & Spider Benchmark & 248 & 446 & 174& 166 & - & - \\ \hline
        
        EX & Chat-SQL  & 221/248 & 331/446& 101/174& 72/166 & 70.1\% & 3\\ 

         % & C3 & - & 224  & 369 & 132 & 99  & 79.7\% \\ 

         & DIN-SQL & 228/248  & 382/446 & 132/174 & 101/166  & 81.5\% & 2\\ 
         
         & DAIL-SQL & 226/248  & 392/446 & 132/174 & 104/166  & 82.6\% & 1\\ 
        \hline

        \hline
        ChatGPT & Chat-SQL & 223/248 & 397/446& 149/174 & 128/166& 86.8\% & 3\\ 
        
         & DIN-SQL & 228/248 & 391/446 & 153/174 & 133/166  & 87.5\%  & 2\\ 
         
         & DAIL-SQL & 235/248  & 407/446 & 158/174 & 142/166 & 91.1\% & 1 \\ 
        % \hdashline

        \hline
         GPT-4o & Chat-SQL& 226/248 & 328/446 & 129/174 &  104/166& 76.1\% & 3\\  

          & DIN-SQL & 231/248 & 376/446  & 150/174 & 126/166 & 85.4\% & 2 \\

         & DAIL-SQL & 228/248 & 397/446  & 153/174 & 129/166 & 87.7\% & 1 \\ 
        

        \hline
        

    \end{tabular}
    \label{table-nl2sql-eval}
\end{table*}



\subsection{Judging Text-to-SQL Generation}
In this subsection, we investigate whether large language models (LLMs) can effectively assess the quality of text-to-SQL generations. Specifically, we compare our proposed \textit{Explain \& Compare} method with the widely used execution match approach. Additionally, we examine which evaluation metric (i.e., LLM judgments or execution match) aligns more closely with user opinions, providing deeper insights into the effectiveness of these approaches.

We first introduce three state-of-the art text-to-SQL algorithms for the Spider benchmark. 

\begin{itemize}
    \item DAIL-SQL~\cite{gao2023text} ranks the first in Spider leader board. DAIL-SQL has extensively investigated different prompting style and few shot selection strategies. It uses GPT-4 with few shot prompting and self-consistency~\cite{wang2022self} to achieve high execution accuracy.

    \item DIN-SQL~\cite{pourreza2023din} ranks the fourth in the leader board and it decompose the text-to-SQL translation problem into sub tasks such as schema linking and classifying the level of difficulties. DIN-SQL uses the GPT-4 model with few-shot prompting.

    \item Chat-SQL~\cite{huang2023chatgpt} directly generate queries using GPT-3.5-Turbo with the zero-shot basic prompt.
\end{itemize}



In Table~\ref{table-nl2sql-eval}, we present the breakdown of the alignment between human preference and the \textit{execution match} and the \textit{LLM judgment} using \textit{Explain \& Compare} prompt on the SQL pairs (gold SQL from Spider and generated SQL from Chat, DIN, and DAIL).


First, we observe that the relative ranking among Chat-SQL, DIN-SQL, and DAIL-SQL remains consistent when transitioning from execution match accuracy to LLM-based evaluations. Given that Chat-SQL relies on SQL queries generated by the weaker model, GPT-3.5-Turbo, using zero-shot prompting, it is expected that the SQL queries produced by DIN-SQL and DAIL-SQL would demonstrate higher accuracy. Furthermore, DAIL-SQL stands out by extensively exploring various prompting techniques for text-to-SQL translation, employing the most effective combination of strategies, and incorporating resource-intensive self-consistency methods. As a result, DAIL-SQL is more likely to generate the most accurate responses. As shown in Table~\ref{table-nl2sql-eval}, the ranking among Chat-SQL, DIN-SQL, and DAIL-SQL based on execution accuracy, GPT-3.5-Turbo judgments, and GPT-4o judgments with our proposed \textit{Explain \& Compare}, all aligned with our expectation.

Additionally, when we examine the accuracy across different difficulty levels (i.e., easy, medium, hard, and extra) in the Spider benchmark, it becomes evident that the primary discrepancies between the execution metric and the LLMs' judgment metric arise from questions classified as hard and extra difficulty. LLMs' judgments, based on the pragmatic equivalence, are less strict than the execution match metric. Consider the following example, \textit{order by col asc/desc limit 1} v.s. \textit{where col = select min/max(col)}. LLMs using \textit{Explain \& Compare} prompt are able to identify the pragmatic equivalence between these two queries (i.e., identifying the top/bottom results based on col) despite their syntactic differences. However, since execution match strictly checks the outputs, it may sometimes return equivalent and other times return not equivalent depending on the underlying database (i.e., whether there are duplicate records sharing the same maximum or minimal value).

\begin{table}[t]
    \centering
    \caption{We compare the agreement between LLMs' judgements and execution matches.}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|l|l}
        {\bf Judge}         & {\bf Data} & {\bf Agreement} \\ \hline
        \multirow{3}{*}{GPT-3.5-Turbo} & Chat-SQL         &     75.8\%       \\ 
        & DIN-SQL         &   83.4\%         
        \\
        & DAIL-SQL         & 85.5\%\\ \hline
        \multirow{3}{*}{GPT-4o}        & Chat-SQL         &   82.6\%               \\ 
        & DIN-SQL         &     87.2\%        
        \\
        & DAIL-SQL         & 89.5\% \\ \hline
    \end{tabular}
    \label{table-agreement}
\end{table}

\subsubsection{Agreement between LLMs' Judgments and Execution Accuracy}

For the majority of questions, the judgments made by large language models (LLMs) align well with execution-based (EX) accuracy. Specifically, as shown in Table~\ref{table-agreement}, the agreement rates between LLMs' judgments (based on pragmatic equivalence) and execution accuracy range from 76\% to 90\%. This strong alignment is an encouraging signal, reflecting both the quality of the Spider benchmark and the reliability of LLMs' judgments. The Spider benchmark is renowned for its high-quality databases, developed with significant human effort—approximately 1,000 hours invested in their creation~\cite{yu2018spider}. This meticulous design ensures the databases are robust, enabling execution-based metrics to produce reliable results. The benchmark's reputation has been widely celebrated within the community for setting a standard in text-to-SQL evaluation.

However, creating such high-quality databases is resource-intensive and does not easily scale, limiting the broader applicability of execution-based metrics. In this context, the high agreement between execution accuracy and LLM-based judgments is particularly desirable. It suggests that LLMs, when guided by pragmatic equivalence, can provide a scalable and reliable alternative for evaluating query accuracy, reducing the dependence on expensive database creation while maintaining strong evaluation standards.



\subsubsection{Alignment with Human Preference}

While LLM judgments and execution-based metrics agree on the majority of questions, there remain many instances where their evaluations diverge. In this subsection, we analyze which metric, LLM judgments or execution accuracy, better aligns with human preferences. By examining these discrepancies, we aim to uncover the strengths and weaknesses of each evaluation approach in accurately assessing the quality of text-to-SQL systems.

\begin{table}[t]
    \centering
     \caption{We compare the human preference between LLM judge, using \textit{Explain \& Compare} prompt and execution match on 70 selected queries from the outputs of text-to-SQL algorithms.}
     
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|l|l}
        {\bf Judge}         & {\bf Few Shot} & {\bf Human Prefer} \\ \hline
        Execution Match & - & 40.0\%
        \\ \hline
        \multirow{2}{*}{GPT-3.5-Turbo} & 0 Shot         &    72.9\%          \\ 
        & 5 Shot         &  74.3\%          \\ \hline
        \multirow{2}{*}{GPT-4o}        & 0 Shot         &    68.6\%                \\ 
        & 5 Shot         &    78.6\%          \\ 
    \end{tabular}
   
    \label{table: human alignment}
\end{table}

\textbf{Human Preferences}
To evaluate the pragmatic equivalence between two SQL queries in text-to-SQL service, we use the human preference approach. Higher alignment to human preference indicates better judgment. At least three experts in SQL have manually checked the equivalence of the 70 selected queries from the state-of-the-art text-to-SQL algorithms~\cite{pourreza2023din, gao2023text, huang2023chatgpt}. These 70 questions include 9 easy questions, 27 medium questions, 14 hard questions, and 20 extra-hard questions. They were randomly selected from cases where an LLM's judgment disagreed with the execution match metric. To ensure the quality of human judgment, the annotations are conducted independently, and we use the majority vote to determine the final label for each pair of SQL queries. 




% When using the semantic equivalence notion, we find GPT 3.5 Turbo may not deliver better judgment than EX, but GPT 4 Turbo results in better alignments. When EX detects discrepancy in the SQL queries' outputs, it often indicates these two SQL queries are not semantically equivalent. There are a few rare cases that we observed in which the SQL queries are semantically equivalent but EX determines not equivalent. For example, when the provided database in Spider contains column values that can not be decoded (similar issues are also raised~\cite{spiderissue}, semantically equivalent queries can be misclassified by EX. 

In Table~\ref{table: human alignment}, we find that execution match only aligned 40\% of the time with human preferences. When using the \textit{Explain \& Compare} prompt for determining the pragmatic equivalence, LLMs are consistently better aligned with human preference than execution match, as shown in Table~\ref{table: human alignment}. The pragmatic notion aims to illustrate the degree to which humans perceive two queries as being similar in their meaning and intent, mimicking the opinions of text-to-SQL users. By reasoning into the query logic and determine whether the two SQL queries share the same logic and have the same intent, LLMs' judgments become better aligned with human preference than execution accuracy. Moreover, when five static examples are included in the prompt, GPT-3.5-Turbo aligned with human preference 74.3\% and GPT-4o aligned with human preference 78.6\%. The positive results on the alignment between LLMs' judgments with human preferences indicate optimizing accuracy for LLMs' judgments is a better optimization target than EX.

Diving deeper into the questions where LLMs failed to align with human preferences, we find that these questions often lack unanimous agreement among experts, as the definition of pragmatic equivalence can be highly subjective. For instance, consider the following two SQL queries:\\

\lstinputlisting[style=SQLStyle]{examples.m}


The queries differ in their filtering criteria: the first uses the airport name to filter for 'Alton', while the second uses the airport code to filter for 'Alton'. Among experts, two considered these queries pragmatically inequivalent, as the filtering criteria are based on different attributes, which could yield totally different output. However, one expert judged them to be pragmatically equivalent, as they have the same intent of finding location based on predicate 'Alton'. LLMs, failing to converge to the majority opinion, interpreted these queries as having the same meaning, possibly oversimplifying the nuanced distinctions in their semantic intent. An exciting avenue for future research is to develop customizable text-to-SQL evaluation metrics tailored to individual user preferences, leveraging in-context learning to adapt the system's understanding and judgments based on specific user requirements or domain contexts.


==> old/approach.tex <==
\section{Proposed Method}
Motivated by recent methods~\cite{deng2023rephrase, yao2023tree, wei2022chain}, we present our prompting techniques to obtain high quality judgments from Open-AI GPT models. Our prompting technique adheres to key aspects widely adopted in NL2SQL 
%liunan2023enhancing
works~\cite{li2023can, khatry2023words, liu2023comprehensive, taori2023stanford}: 1) \textbf{Clear Layout}: We provide the instruction at the beginning, followed by the two SQL queries that need to be compared, and end by providing the database schema. 2) \textbf{Clear Context}: We provide the database schema and explicitly included the primary and foreign key constraints, since they are crucial context information for deciding SQL equivalence. 

For semantic equivalence, we also added a short definition of SQL semantic equivalence (i.e., \textit{Note: Two SQL queries are semantically equivalent if and only if they yield identical results for all possible databases.}). In addition, we first ask GPT to generate a counter example if there exists one and then decide if two SQL queries are equivalent. We call this prompt the \textbf{Counter Example} prompt. However, as shown in Figure~\ref{fig:llm prompt}, the counter example prompt leads to sub-optimal results, especially when GPT models only scratched the surface and observed the obvious (similarity between two SQL queries in structure and logic). This finding aligns with the prior works~\cite{wang2023large, zheng2023judging} which demonstrated that GPT models exhibit bias toward ignoring small differences when determining SQL equivalence and exhibit limited reasoning capability.

To overcome this observed phenomenon, we introduce our proposed prompting technique in detail to obtain better responses from large language models. In complex problem solving, people always start with a simple example and then introduce more complex elements to understand the full picture. Motivated by this simple intuition, we incorporate this idea and proposed the \textbf{Miniature and Mull} prompting technique. In particular, we first ask GPT to execute both queries on a simple database and then see if it can modify the database such that the two queries output different results (i.e., a counter example). As shown later in the experimental section, this approach can directly enhance the LLM’s response accuracy in determining SQL semantic equivalence. We believe that this prompting technique has wide applications in comparing the equivalence of two codes, plans, and logic.

For relaxed equivalence, we designed the \textbf{Explain and Compare} prompt by asking the LLMs to perform multi-step reasoning before determining if the two SQL queries are equivalent. This prompt follows the main ideas from the chain-of-thoughts~\cite{wei2022chain}. We first prompt the LLMs to explain two SQL queries and then ask it to determine if these two queries contain significant difference in logic, as shown in Figure~\ref{fig:llm prompt}. We observe that LLMs are inclined to label two SQL queries as equivalent when they appear similar in structure. As a result, it is crucial for LLMs to be able to first spot the differences between these two queries and then apply this knowledge in considering if these two SQL queries are relaxed equivalent.

%We find GPT inherent incline to answer equivalent for two similar SQL queries. Since OpenAI LLMs seems to implicitly take the relaxed notion of equivalence, we directly use the chain of thought appraoch.


==> old/background.tex <==
\section{Background}

\subsection{Motivations}
We first introduce a query rewriting error that happened in the real-world system, known as the COUNT bug~\cite{ganski1987optimization}. Here are two SQL queries Q1 and Q2 as shown below:

\lstinputlisting[language=Octave]{CountBug.m}

One may think these two queries are equivalent, since they both return results based on the condition that \textbf{qoh} from \textbf{Supply} table equals to the counts of records in the \textbf{Supply} table when \textbf{shipdate} is less than 10; however they are different in how they handle the subquery. Suppose that there is a record $R$ in the \textit{Parts} table such that \textit{R.qoh} is zero and \textit{R.pnum} does not exist in the \textit{Supply} table. 
Then, Q1 will include record $R$ since \textit{R.qoh} is zero and selecting the count for \textit{R.pnum} from the \textit{Supply} table will also return zero. On the other hand, Q2 will not include record $R$ because the \textit{TEMP} result will not contain \textit{R.pnum}. 


% When asked to provide a counterexample, it is able to generate a counterexample in which it provides a database instance containing such a record $R$ as described above. 
Hence, real-world data systems need tools to avoid such pitfalls. While proving the semantic equivalency between two SQL queries has been proved to be undecidable~\cite{trahtenbrot1963impossibility, libkin2004elements, sagiv1980equivalences}, we believe LLMs may offer new opportunities to help data engineers in scrutinizing their SQL optimization logic and potentially identify flaws accordingly. For instance, when we present the COUNT BUG to ChatGPT, ChatGPT is able to correctly identify that these two SQL queries are not equivalent. 


\textcolor{black}{Moreover, in text-to-SQL generation, many natural language questions are inherently ambiguous~\cite{katsogiannis2023survey, Floratou2024NL2SQL}, and as a result, they can be interpreted and answered in multiple ways~\cite{min2020ambigqa}. From the user's perspective, different SQL queries that convey the same logical answer to a question may all be considered equivalent. However, the widely used \textit{execution match} metric, which expects a single correct SQL query, does not capture these ambiguities. Consequently, we are interested in exploring whether LLMs can be utilized to assess the quality of text-to-SQL generation.}

% \begin{figure}
%     \centering
%     \includegraphics{figures/CountBug.PNG}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

\subsubsection{Two Notions of SQL Equivalence}
Motivated from the query optimizers in data systems and evaluation metrics for text-to-SQL, we define two notions of SQL equivalence.

\begin{definition}[Semantic Equivalence]~\label{formal-view}
Two SQL queries Q1 and Q2 are said to be {\em semantically equivalent} if and only if there does not exist a database instance such that Q1 and Q2 return different outputs.
\end{definition}

\begin{definition}[Relaxed Equivalence]~\label{human-view}
Two SQL queries Q1 and Q2 are said to be {\em relaxed equivalent} if one may edit a trivial portion of the SQL queries while preserving the same logic to make Q1 and Q2 semantically equivalent.
\end{definition}

% Based on the semantic definition of SQL equivalence (Definition~\ref{formal-view}), the Count bug is indeed a flaw for query engines and should be remedied immediately. On the other hand, we argue that based on Definition~\ref{human-view}, which reflects the logical perspective and aligned with human perception, the two SQL queries in the Count Bug example are relaxed logically equivalent. The fact that even experienced experts failed to identify this subtle difference indicates humans often recognize equivalence based on the relaxed notion, and the relaxed notion of equivalence can better capture a human user's satisfaction with the generated SQL from foundational models. 


% To illustrate why these two queries are relaxed logically equivalent, Q2 in the Count Bug example only the \textit{TEMP} table needs to be edited as shown below for it to be semantically equivalent to Q1 in the Count Bug example:
% \lstinputlisting[language=Octave]{Q2Edit.m}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figures/LLM-Solver-Prompts.pptx.jpg}
    \caption{Demonstration of Counter Example, Miniature \& MULL, and Explain \% Compare prompts. The used SQL queries are not semantically equivalent but are relaxed equivalent.}
    \label{fig:llm prompt}
\end{figure*}

\subsection{Why LLM-SQL-Solver}
First, LLM-SQL-Solver (semantic notion) can be directly used to find system bugs (e.g., COUNT BUG) and help engineers validate their SQL rewriting code bases. Second, since query optimizer relies on heuristic rules to find equivalent SQL forms, it may not explore all rewriting possibilities and hence, the rewritten query may lead to sub optimal performance. We believe that, with LLM-SQL-Solver, query optimizers can explore the vast universe of equivalent rewritten queries and then find the query plan with near optimal performance.

For text-to-SQL tasks, we believe that when comparing the gold SQL query (the correct answer) with the generated SQL query, the current most popular metric, \textit{execution match}, does not reflects the human perspective and fails to capture a user's opinion on the generated SQL. For instance, a common reasoning for failures in \textit{execution match} is that the generated SQL selects fewer/extra columns than the gold SQL. In fact, a recent work has explicitly added \textit{"do not select extra columns"} in its prompt to improve the execution accuracy~\cite{dong2023c3}. However, from a user's perspective providing extra columns may not reduce the quality of the answer. Also, there are many other similar reasons that can lead to false execution matches but not necessarily indicate a lower quality of the generated SQL query (such as the column order in selection, case sensitivity, duplicate entries, and columns in different tables share the similar contents). 
Moreover, execution matching fails to correctly identify logically different queries when the underlying database does not contain any counter examples, even when hundreds of human hours were consumed to create the benchmark~\cite{yu2018spider}. Lastly, a fundamental limitation of execution accuracy is its need to query the underlying database. This is particularly pertinent as the text-to-SQL service provider usually does not have ownership of the user's database and the user’s database may also contain sensitive information. 
As a result, it would be desirable to have a SQL solver determining the relax notion of equivalence without constructing sophisticated databases and without accessing any stored data. Hence, in additional to investigating the capability of foundational models in identifying semantic equivalence, we further explore whether LLM-SQL-Solver (relaxed notion) can be used as a better metric for text-to-SQL benchmarks.

% As a result, in this paper, we would like to mainly answer the following questions: 
% \begin{itemize}
%     \item Can LLMs help data engineers in identifying SQL semantic equivalence?
%     \item Should LLMs be used to evaluate the quality of generated SQL queries?
% \end{itemize}


==> old/conclusion.tex <==
\section{Conclusion}
In this paper, we studied and answered two main questions: i) Can current LLMs be used to help engineers in checking semantic equivalences between SQL queries and ii) should we use LLMs to judge the quality of generated SQL queries for text-to-SQL benchmarks. To the best of our knowledge, this is the first work studying the ability of LLMs in understanding SQL queries and determining SQL equivalences. Through extensive evaluations and manually examining the quality of the answers based on the alignment with human preferences, we find current LLMs (especially GPT 4 turbo), using our proposed prompt techniques, can assists engineers in determining semantic equivalent queries, but may yield incorrect responses. On the other hand, when comparing the generated SQL query with the gold SQL query with our relaxed notion of equivalence, LLMs' responses constantly achieve high alignments with human preferences. Moreover, our proposed LLM-SQL-Solver avoids accessing stored user data, and hence no sophisticated databases need to be constructed.

 
 % As the learning ability in LLMs continuously to advance, we believe that using these models to check SQL equivalence is a promising direction.


% Another critical advantage of using LLMs to determine SQL equivalence is that it can avoid the construction of sophisticated databases, and no data stored need to be accessed. 


==> old/discussion.tex <==
\section{Discussion and Limitation}
In this discussion section, we would like to highlight the broader implications and potential integration of our proposed LLM-SQL-Solver. 
During the SQL rewrite phase of the query optimization engine, the input SQL query is transformed into a new SQL query that can be optimized more easily. The key challenge in query rewriting is to determine if the input query and the rewritten query are indeed semantic equivalent. The LLM-SQL-Solver can be directly used as a tool, during the rewriting phase, to check semantic equivalence and ensure bugs (e.g., COUNT bug~\cite{ganski1987optimization}) do not occur in the data system. Furthermore, the integration of the LLM-SQL-Solver as a text-to-SQL evaluation metrics using the relaxed equivalence notion could improve the overall quality of user experience and enable more human-like capabilities.

\textcolor{black}{Concurrent with our research, the chain-of-table approach~\cite{wang2024chain} independently explores a similar concept, allowing LLMs to form a reasoning path through table modifications to improve question answering from tabular data, akin to our \textit{Miniature \& Mull} prompt. However, while our technique focuses on determining query semantic equivalence through table creation and modification, their goal is to deepen the understanding of the tabular data itself.}
% Snowflake~\cite{snowflake} has also independently determined that LLMs' judgments serve as a more effective optimization target for evaluating text-to-SQL generation. Similarly,

There are some limitations or areas of improvement to this work. First, we only evaluated the capabilities of the Large Language Models of OpenAI. There are other alternative models such as Llama2 7B~\cite{touvron2023llama}, Vicuna~\cite{chiang2023vicuna}, Alpaca~\cite{taori2023alpaca} which also showcase strong understanding and reasoning for logical tasks~\cite{chen2021evaluating, yue2023mmmu, yan2023codetransocean}. Nevertheless, we believe that GPT 3.5 turbo and GPT 4 turbo exemplify the current status of the GPT model family's capabilities. 
In addition, our evaluations on Spider Benchmark were conducted over randomly sampled questions, in which we have to manually label the equivalence of the two different notions (semantic and relaxed).
Since there are nearly ten thousand pairs of SQL queries, manually checking all of them are arguably infeasible. In fact, even checking a pair of SQL queries for semantic view takes around 10 minutes for experts in SQL. Although the questions are sampled, we observe a consistent trends between LLMs' judgements and execution matches (such as GPT 4 turbo's responses are consistently better aligned with human preferences).

==> old/intro.tex <==
\section{Introduction}
Structured Query Language (SQL) it is the standard programming language to query data systems and it is one of the most popular programming language~\cite{sqlpopular}. Since SQL is not a procedural language, one may write different SQL queries that are semantically equivalent. As a result, determining the equivalence of SQL queries is a fundamental task in many practical important applications ranging from query optimizers in database systems~\cite{pirahesh1992extensible, bai2023querybooster, zhou2021learned, samwel2018f1} to evaluating the translation from user text-to-SQL~\cite{zelle1996learning, zhong2020grounded, khatry2023words, cidrsql}. However, it has been shown by the data management research community that checking the equivalence of two SQL queries is in general undecidable~\cite{abiteboul1995foundations}. While there are theoretical works to check equivalence under different assumptions~\cite{chandra1977optimal, sagiv1980equivalences, cohen1999rewriting, chu2018axiomatic} and implemented prototypes such as Cosette~\cite{chu2017cosette}, they only support limited SQL operations and such projects are no longer maintained due to lack of experts. For instance, Cosette does not support commonly found operations like \textit{EXISTS}, \textit{IN}, queries with constant expressions, etc.; and Cosette is no longer maintained due to the lack of staff. Query optimizers and query processing engines in data systems still primarily rely on heuristic query rewriting rules~\cite{begoli2018apache}. Exploring and writing these rules correctly require strong domain expertise and need many engineering hours.

Moreover, due to the difficulty in evaluating the equivalence of two SQL queries, Text-to-SQL literature~\cite{zhong2017seq2sql, yu2018spider, wang2019rat, lee2021kaggledbqa, li2023can} primarily use \textit{exact match} (exact SQL string match) or \textit{execution match} (compare the execution outputs) as the evaluation metrics. However, exact string match may overlook many equivalent SQL queries (there are many ways different ways to write the same SQL query), and \textit{execution match} may misclassify different SQL queries as equivalent due to the lack of counterexamples in the underlining database instance. \textcolor{black}{We note that there have been a few attempts that explore using semantic equivalence as the evaluation metrics~\cite{zhong2020semantic}. These methods assess query semantic equivalence by generating numerous fuzzy database instances, leading to significant computational and storage demands. Specifically, evaluating a thousand pairs of SQL queries requires at least 75 minutes and consumes about 3 GB of storage space for creating these fuzz database instances~\cite{zhong2020semantic}.}

Recent advancements in large language models (LLMs) have shown great capability in following instructions and in generating decisions that align with human judgement~\cite{bubeck2023sparks, chiang2023can, yan2023codescope, zhang2023gpt}. For instance, It has been shown that GPT models are capable of performing first order logic reasoning~~\cite{saparov2022language}, detecting implicit contents~\cite{huang2023chatgpt, zhang2023schema}, and solving complex logical problems~\cite{feng2023language, yao2023tree}. In this paper, we investigate whether LLM can act as a judge to determine the equivalence of SQL queries. Hence, in this paper, we would like to mainly answer the following questions: 
\begin{itemize}
    \item Can LLMs help data engineers in identifying SQL semantic equivalence?
    \item Should LLMs be used to evaluate text-to-SQL generation?
\end{itemize}


